Surrogate-based optimization of system architectures subject to hidden constraints

The exploration of novel architectures requires physics-based simulation due to a lack of prior experience to start from, which introduces two specific challenges for optimization algorithms: evaluations become more expensive (in time) and evaluations might fail. The former challenge is addressed by Surrogate-Based Optimization (SBO) algorithms, in particular Bayesian Optimization (BO) using Gaussian Process (GP) models. An overview is provided of how BO can deal with challenges specific to architecture optimization, such as design variable hierarchy and multiple objectives: specific measures include ensemble infills and a hierarchical sampling algorithm. Evaluations might fail due to non-convergence of underlying solvers or infeasible geometry in certain areas of the design space. Such failed evaluations, also known as hidden constraints, pose a particular challenge to SBO/BO, as the surrogate model cannot be trained on empty results. This work investigates various strategies for satisfying hidden constraints in BO algorithms. Three high-level strategies are identified: rejection of failed points from the training set, replacing failed points based on viable (non-failed) points, and predicting the failure region. Through investigations on a set of test problems including a jet engine architecture optimization problem, it is shown that best performance is achieved with a mixed-discrete GP to predict the Probability of Viability (PoV), and by ensuring selected infill points satisfy some minimum PoV threshold. This strategy is demonstrated by solving a jet engine architecture problem that features at 50% failure rate and could not previously be solved by a BO algorithm. The developed BO algorithm and used test problems are available in the open-source Python library SBArchOpt.

==> figures/exp_03_04a_min_pov/rank.tex <==
\begin{tabular}{llccccccccccc}
\toprule
 & Alimo & Alimo Edge & Müller 1 & MD/HC Carside & H Alimo & H/HC Rbr. & MO/H/HC Rbr. & Jet SM & Rank 1 & Rank $\leq$ 2 & Penalty \\
Strategy & Config &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
Predicted Worst & $\alpha = 1.00$ & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{AEDEA7}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{AEDEA7}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{C6DBEF}} \color[HTML]{000000} 25\% & {\cellcolor[HTML]{2070B4}} \color[HTML]{F1F1F1} 75\% & {\cellcolor[HTML]{2A924A}} \color[HTML]{F1F1F1} 15\% \\
Predicted Worst & $\alpha = 1.50$ & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{AEDEA7}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{9DCAE1}} \color[HTML]{000000} 38\% & {\cellcolor[HTML]{08509B}} \color[HTML]{F1F1F1} 88\% & {\cellcolor[HTML]{218944}} \color[HTML]{F1F1F1} 13\% \\
Predicted Worst & $\alpha = 2.00$ & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{AEDEA7}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{AEDEA7}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{DEEBF7}} \color[HTML]{000000} 12\% & {\cellcolor[HTML]{4191C6}} \color[HTML]{F1F1F1} 62\% & {\cellcolor[HTML]{B0DFAA}} \color[HTML]{000000} 36\% \\
\underline{MD-GP} & \underline{$f_{infill}$ penalty} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{2070B4}} \color[HTML]{F1F1F1} \underline{75\%} & {\cellcolor[HTML]{08306B}} \color[HTML]{F1F1F1} \underline{100\%} & {\cellcolor[HTML]{00491D}} \color[HTML]{F1F1F1} \underline{1\%} \\
MD-GP & $PoV_{min} = 10\%$ & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4191C6}} \color[HTML]{F1F1F1} 62\% & {\cellcolor[HTML]{08306B}} \color[HTML]{F1F1F1} 100\% & {\cellcolor[HTML]{005723}} \color[HTML]{F1F1F1} 3\% \\
\underline{MD-GP} & \underline{$PoV_{min} = 25\%$} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{2070B4}} \color[HTML]{F1F1F1} \underline{75\%} & {\cellcolor[HTML]{08306B}} \color[HTML]{F1F1F1} \underline{100\%} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{-1\%} \\
MD-GP & $PoV_{min} = 50\%$ & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4191C6}} \color[HTML]{F1F1F1} 62\% & {\cellcolor[HTML]{08509B}} \color[HTML]{F1F1F1} 88\% & {\cellcolor[HTML]{0C7735}} \color[HTML]{F1F1F1} 9\% \\
MD-GP & $PoV_{min} = 75\%$ & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{AEDEA7}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 50\% & {\cellcolor[HTML]{08509B}} \color[HTML]{F1F1F1} 88\% & {\cellcolor[HTML]{026F2E}} \color[HTML]{F1F1F1} 7\% \\
MD-GP & $PoV_{min} = 90\%$ & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 50\% & {\cellcolor[HTML]{08509B}} \color[HTML]{F1F1F1} 88\% & {\cellcolor[HTML]{208843}} \color[HTML]{F1F1F1} 13\% \\
RFC & $f_{infill}$ penalty & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{AEDEA7}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4191C6}} \color[HTML]{F1F1F1} 62\% & {\cellcolor[HTML]{08509B}} \color[HTML]{F1F1F1} 88\% & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} -2\% \\
RFC & $PoV_{min} = 10\%$ & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{AEDEA7}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{9DCAE1}} \color[HTML]{000000} 38\% & {\cellcolor[HTML]{08509B}} \color[HTML]{F1F1F1} 88\% & {\cellcolor[HTML]{107A37}} \color[HTML]{F1F1F1} 10\% \\
RFC & $PoV_{min} = 25\%$ & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 50\% & {\cellcolor[HTML]{08306B}} \color[HTML]{F1F1F1} 100\% & {\cellcolor[HTML]{006729}} \color[HTML]{F1F1F1} 6\% \\
RFC & $PoV_{min} = 50\%$ & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{AEDEA7}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 50\% & {\cellcolor[HTML]{08509B}} \color[HTML]{F1F1F1} 88\% & {\cellcolor[HTML]{004C1E}} \color[HTML]{F1F1F1} 1\% \\
RFC & $PoV_{min} = 75\%$ & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{9DCAE1}} \color[HTML]{000000} 38\% & {\cellcolor[HTML]{08306B}} \color[HTML]{F1F1F1} 100\% & {\cellcolor[HTML]{0E7936}} \color[HTML]{F1F1F1} 9\% \\
RFC & $PoV_{min} = 90\%$ & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{AEDEA7}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{37A055}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{AEDEA7}} \color[HTML]{000000} 3 & {\cellcolor[HTML]{DEEBF7}} \color[HTML]{000000} 12\% & {\cellcolor[HTML]{9DCAE1}} \color[HTML]{000000} 38\% & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} 54\% \\
\bottomrule
\end{tabular}


==> figures/exp_03_05_opt/rank.tex <==
\begin{tabular}{lcccccccccc}
\toprule
 & Branin & HC Branin & Alimo & Alimo Edge & Müller 2 & HC Sphere & Müller 1 & HC CantB & HC Carside Less & HC Carside \\
\midrule
Rejection &  & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 5 & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} 6 & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} 6 \\
Replacement & Global max & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 5 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 \\
Replacement & Local & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 5 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 5 \\
Replacement & 5-nearest, max & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 \\
Replacement & 5-nearest, mean & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 \\
Replacement & Predicted worst & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 \\
Replacement & Pred. worst ($\alpha = 2$) & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 \\
\underline{Prediction} & \underline{RFC} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} \underline{3} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} \\
Prediction & KNN & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 \\
Prediction & RBF & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 \\
Prediction & GP Classifier & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 \\
Prediction & Variational GP & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 \\
Prediction & MD GP & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 \\
\bottomrule
\end{tabular}
\vspace{15pt}
\begin{tabular}{cccccccccc}
\toprule
MD/HC CantB & MD/HC Carside & H Alimo & H Alimo Edge & H Müller 2 & H/HC Rosenbr. & MO/H/HC Rbr. & Jet SM & Rank 1 & Rank $\leq$ 2 \\
\midrule
{\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 5 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{E1EDF8}} \color[HTML]{000000} 11\% & {\cellcolor[HTML]{ABD0E6}} \color[HTML]{000000} 33\% \\
{\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 5 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{E1EDF8}} \color[HTML]{000000} 11\% & {\cellcolor[HTML]{82BBDB}} \color[HTML]{000000} 44\% \\
{\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{ECF4FB}} \color[HTML]{000000} 6\% & {\cellcolor[HTML]{99C7E0}} \color[HTML]{000000} 39\% \\
{\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{CCDFF1}} \color[HTML]{000000} 22\% & {\cellcolor[HTML]{3787C0}} \color[HTML]{F1F1F1} 67\% \\
{\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{99C7E0}} \color[HTML]{000000} 39\% & {\cellcolor[HTML]{105BA4}} \color[HTML]{F1F1F1} 83\% \\
{\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{58A1CF}} \color[HTML]{F1F1F1} 56\% & {\cellcolor[HTML]{105BA4}} \color[HTML]{F1F1F1} 83\% \\
{\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{99C7E0}} \color[HTML]{000000} 39\% & {\cellcolor[HTML]{2979B9}} \color[HTML]{F1F1F1} 72\% \\
{\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} \underline{78\%} & {\cellcolor[HTML]{083E81}} \color[HTML]{F1F1F1} \underline{94\%} \\
{\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{D6E6F4}} \color[HTML]{000000} 17\% & {\cellcolor[HTML]{3787C0}} \color[HTML]{F1F1F1} 67\% \\
{\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{6AAED6}} \color[HTML]{F1F1F1} 50\% & {\cellcolor[HTML]{105BA4}} \color[HTML]{F1F1F1} 83\% \\
{\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4695C8}} \color[HTML]{F1F1F1} 61\% & {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 78\% \\
{\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{58A1CF}} \color[HTML]{F1F1F1} 56\% & {\cellcolor[HTML]{1B69AF}} \color[HTML]{F1F1F1} 78\% \\
{\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 5 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{2979B9}} \color[HTML]{F1F1F1} 72\% & {\cellcolor[HTML]{083E81}} \color[HTML]{F1F1F1} 94\% \\
\bottomrule
\end{tabular}


==> figures/exp_03_05_opt/rank_mod_old.tex <==
\begin{tabular}{llccccccccc}
\toprule
& & Branin & HC Branin & Alimo & Alimo Edge & Müller 2 & HC Sphere & Müller 1 & HC CantB & HC Carside Less \\
\midrule
Rejection &  & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 5 \\
Replacement & Global max & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 \\
Replacement & Local & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 \\
Replacement & 5-nearest, max & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 \\
Replacement & 5-nearest, mean & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 \\
Replacement & Predicted worst & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 \\
Replacement & Pred. worst ($\alpha = 2$) & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 \\
\underline{Prediction} & \underline{RFC} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} \underline{2} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} \underline{2} \\
Prediction & KNN & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 \\
Prediction & RBF & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 \\
Prediction & GP Classifier & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 \\
Prediction & Variational GP & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 \\
Prediction & MD GP & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 \\
\bottomrule
\vspace{15pt}
\end{tabular}
\begin{tabular}{cccccccccc}
\toprule
HC Carside & MD/HC CantB & MD/HC Carside & H Alimo & H Alimo Edge & H Müller 2 & H/HC Rosenbr. & MO/H/HC Rbr. & Rank 1 & Rank $\leq$ 2 \\
\midrule
{\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} 6 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 5 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{D4E4F4}} \color[HTML]{000000} 18\% & {\cellcolor[HTML]{8FC2DE}} \color[HTML]{000000} 41\% \\
{\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{A5CDE3}} \color[HTML]{000000} 35\% & {\cellcolor[HTML]{3C8CC3}} \color[HTML]{F1F1F1} 65\% \\
{\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 5 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{DFECF7}} \color[HTML]{000000} 12\% & {\cellcolor[HTML]{B8D5EA}} \color[HTML]{000000} 29\% \\
{\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{B8D5EA}} \color[HTML]{000000} 29\% & {\cellcolor[HTML]{125EA6}} \color[HTML]{F1F1F1} 82\% \\
{\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{D3EECD}} \color[HTML]{000000} 5 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{A5CDE3}} \color[HTML]{000000} 35\% & {\cellcolor[HTML]{084F99}} \color[HTML]{F1F1F1} 88\% \\
{\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{3C8CC3}} \color[HTML]{F1F1F1} 65\% & {\cellcolor[HTML]{08306B}} \color[HTML]{F1F1F1} 100\% \\
{\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{77B5D9}} \color[HTML]{000000} 47\% & {\cellcolor[HTML]{084082}} \color[HTML]{F1F1F1} 94\% \\
{\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} \underline{2} & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} \underline{2} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} \underline{2} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} \underline{1} & {\cellcolor[HTML]{2D7DBB}} \color[HTML]{F1F1F1} \underline{71\%} & {\cellcolor[HTML]{08306B}} \color[HTML]{F1F1F1} \underline{100\%} \\
{\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{98D594}} \color[HTML]{000000} 4 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{A5CDE3}} \color[HTML]{000000} 35\% & {\cellcolor[HTML]{1E6DB2}} \color[HTML]{F1F1F1} 76\% \\
{\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4E9ACB}} \color[HTML]{F1F1F1} 59\% & {\cellcolor[HTML]{125EA6}} \color[HTML]{F1F1F1} 82\% \\
{\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{77B5D9}} \color[HTML]{000000} 47\% & {\cellcolor[HTML]{125EA6}} \color[HTML]{F1F1F1} 82\% \\
{\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4E9ACB}} \color[HTML]{F1F1F1} 59\% & {\cellcolor[HTML]{1E6DB2}} \color[HTML]{F1F1F1} 76\% \\
{\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{157F3B}} \color[HTML]{F1F1F1} 2 & {\cellcolor[HTML]{00441B}} \color[HTML]{F1F1F1} 1 & {\cellcolor[HTML]{4BB062}} \color[HTML]{F1F1F1} 3 & {\cellcolor[HTML]{3C8CC3}} \color[HTML]{F1F1F1} 65\% & {\cellcolor[HTML]{084082}} \color[HTML]{F1F1F1} 94\% \\
\bottomrule
\end{tabular}


==> figures/exp_03_05_opt/rel_perf.tex <==
\begin{tabular}{llccccc}
\toprule
 & $\Delta HV$ regret & Fail rate & Training time & Infill time & Training + infill time \\
names &  &  &  &  &  \\
\midrule
Rejection &  & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} +0\% & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} +0\% & {\cellcolor[HTML]{FFF5F0}} \color[HTML]{000000} +0\% & {\cellcolor[HTML]{FFF5F0}} \color[HTML]{000000} +0\% & {\cellcolor[HTML]{FFF5F0}} \color[HTML]{000000} +0\% \\
Replacement & Global max & {\cellcolor[HTML]{EBF7E7}} \color[HTML]{000000} -9\% & {\cellcolor[HTML]{46AE60}} \color[HTML]{F1F1F1} -61\% & {\cellcolor[HTML]{69000D}} \color[HTML]{F1F1F1} +199\% & {\cellcolor[HTML]{FC9474}} \color[HTML]{000000} +74\% & {\cellcolor[HTML]{FC9373}} \color[HTML]{000000} +74\% \\
Replacement & Local & {\cellcolor[HTML]{E5F5E0}} \color[HTML]{000000} -13\% & {\cellcolor[HTML]{DEF2D9}} \color[HTML]{000000} -15\% & {\cellcolor[HTML]{67000D}} \color[HTML]{F1F1F1} +202\% & {\cellcolor[HTML]{FC9272}} \color[HTML]{000000} +76\% & {\cellcolor[HTML]{FC8B6B}} \color[HTML]{F1F1F1} +79\% \\
Replacement & 5-nearest, max & {\cellcolor[HTML]{B7E2B1}} \color[HTML]{000000} -30\% & {\cellcolor[HTML]{8DD08A}} \color[HTML]{000000} -43\% & {\cellcolor[HTML]{67000D}} \color[HTML]{F1F1F1} +207\% & {\cellcolor[HTML]{FC8D6D}} \color[HTML]{F1F1F1} +78\% & {\cellcolor[HTML]{FC8464}} \color[HTML]{F1F1F1} +84\% \\
Replacement & 5-nearest, mean & {\cellcolor[HTML]{A8DCA2}} \color[HTML]{000000} -35\% & {\cellcolor[HTML]{CDECC7}} \color[HTML]{000000} -23\% & {\cellcolor[HTML]{79040F}} \color[HTML]{F1F1F1} +193\% & {\cellcolor[HTML]{FC8D6D}} \color[HTML]{F1F1F1} +78\% & {\cellcolor[HTML]{FC8F6F}} \color[HTML]{000000} +77\% \\
Replacement & Predicted worst & {\cellcolor[HTML]{AEDEA7}} \color[HTML]{000000} -33\% & {\cellcolor[HTML]{7AC77B}} \color[HTML]{000000} -48\% & {\cellcolor[HTML]{7A0510}} \color[HTML]{F1F1F1} +192\% & {\cellcolor[HTML]{FC9E80}} \color[HTML]{000000} +67\% & {\cellcolor[HTML]{FC9576}} \color[HTML]{000000} +73\% \\
Replacement & Pred. worst ($\alpha = 2$) & {\cellcolor[HTML]{B7E2B1}} \color[HTML]{000000} -30\% & {\cellcolor[HTML]{68BE70}} \color[HTML]{000000} -53\% & {\cellcolor[HTML]{69000D}} \color[HTML]{F1F1F1} +199\% & {\cellcolor[HTML]{FC9373}} \color[HTML]{000000} +75\% & {\cellcolor[HTML]{FC8D6D}} \color[HTML]{F1F1F1} +78\% \\
Prediction & RFC & {\cellcolor[HTML]{8ACE88}} \color[HTML]{000000} -44\% & {\cellcolor[HTML]{48AE60}} \color[HTML]{F1F1F1} -61\% & {\cellcolor[HTML]{FC8060}} \color[HTML]{F1F1F1} +86\% & {\cellcolor[HTML]{FB7353}} \color[HTML]{F1F1F1} +94\% & {\cellcolor[HTML]{FC8565}} \color[HTML]{F1F1F1} +83\% \\
Prediction & KNN & {\cellcolor[HTML]{C2E7BB}} \color[HTML]{000000} -27\% & {\cellcolor[HTML]{9BD696}} \color[HTML]{000000} -39\% & {\cellcolor[HTML]{FCBEA5}} \color[HTML]{000000} +48\% & {\cellcolor[HTML]{FCAD90}} \color[HTML]{000000} +59\% & {\cellcolor[HTML]{FCBDA4}} \color[HTML]{000000} +49\% \\
Prediction & RBF & {\cellcolor[HTML]{A9DCA3}} \color[HTML]{000000} -35\% & {\cellcolor[HTML]{48AE60}} \color[HTML]{F1F1F1} -61\% & {\cellcolor[HTML]{ED392B}} \color[HTML]{F1F1F1} +126\% & {\cellcolor[HTML]{FC7F5F}} \color[HTML]{F1F1F1} +87\% & {\cellcolor[HTML]{FC8A6A}} \color[HTML]{F1F1F1} +80\% \\
Prediction & GP Classifier & {\cellcolor[HTML]{A2D99C}} \color[HTML]{000000} -37\% & {\cellcolor[HTML]{52B365}} \color[HTML]{F1F1F1} -58\% & {\cellcolor[HTML]{F85D42}} \color[HTML]{F1F1F1} +106\% & {\cellcolor[HTML]{C1161B}} \color[HTML]{F1F1F1} +156\% & {\cellcolor[HTML]{F44F39}} \color[HTML]{F1F1F1} +114\% \\
Prediction & Variational GP & {\cellcolor[HTML]{B0DFAA}} \color[HTML]{000000} -32\% & {\cellcolor[HTML]{4AAF61}} \color[HTML]{F1F1F1} -60\% & {\cellcolor[HTML]{FC9E80}} \color[HTML]{000000} +68\% & {\cellcolor[HTML]{67000D}} \color[HTML]{F1F1F1} +243\% & {\cellcolor[HTML]{820711}} \color[HTML]{F1F1F1} +189\% \\
Prediction & MD GP & {\cellcolor[HTML]{A0D99B}} \color[HTML]{000000} -38\% & {\cellcolor[HTML]{45AD5F}} \color[HTML]{F1F1F1} -62\% & {\cellcolor[HTML]{F34C37}} \color[HTML]{F1F1F1} +116\% & {\cellcolor[HTML]{FB7252}} \color[HTML]{F1F1F1} +95\% & {\cellcolor[HTML]{FB7858}} \color[HTML]{F1F1F1} +91\% \\
\bottomrule
\end{tabular}


==> figures/exp_03_05_opt/rel_perf_mod_old.tex <==
\begin{tabular}{llccccc}
\toprule
 Strategy & Sub-strategy & $\Delta HV$ regret & Fail rate & Training time & Infill time & Training + infill time \\
\midrule
Rejection &  & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} +0\% & {\cellcolor[HTML]{F7FCF5}} \color[HTML]{000000} +0\% & {\cellcolor[HTML]{FFF5F0}} \color[HTML]{000000} +0\% & {\cellcolor[HTML]{FFF5F0}} \color[HTML]{000000} +0\% & {\cellcolor[HTML]{FFF5F0}} \color[HTML]{000000} +0\% \\
Replacement & Global max & {\cellcolor[HTML]{D4EECE}} \color[HTML]{000000} -20\% & {\cellcolor[HTML]{3FA95C}} \color[HTML]{F1F1F1} -63\% & {\cellcolor[HTML]{A10E15}} \color[HTML]{F1F1F1} +176\% & {\cellcolor[HTML]{FC7F5F}} \color[HTML]{F1F1F1} +87\% & {\cellcolor[HTML]{F75C41}} \color[HTML]{F1F1F1} +107\% \\
Replacement & Local & {\cellcolor[HTML]{F6FCF4}} \color[HTML]{000000} -1\% & {\cellcolor[HTML]{E1F3DC}} \color[HTML]{000000} -14\% & {\cellcolor[HTML]{A50F15}} \color[HTML]{F1F1F1} +174\% & {\cellcolor[HTML]{FB6B4B}} \color[HTML]{F1F1F1} +99\% & {\cellcolor[HTML]{F7593F}} \color[HTML]{F1F1F1} +109\% \\
Replacement & 5-nearest, max & {\cellcolor[HTML]{ACDEA6}} \color[HTML]{000000} -34\% & {\cellcolor[HTML]{84CC83}} \color[HTML]{000000} -46\% & {\cellcolor[HTML]{AB1016}} \color[HTML]{F1F1F1} +171\% & {\cellcolor[HTML]{FB7C5C}} \color[HTML]{F1F1F1} +89\% & {\cellcolor[HTML]{FA6648}} \color[HTML]{F1F1F1} +102\% \\
Replacement & 5-nearest, mean & {\cellcolor[HTML]{B2E0AC}} \color[HTML]{000000} -32\% & {\cellcolor[HTML]{C3E7BC}} \color[HTML]{000000} -26\% & {\cellcolor[HTML]{A50F15}} \color[HTML]{F1F1F1} +174\% & {\cellcolor[HTML]{FB7757}} \color[HTML]{F1F1F1} +92\% & {\cellcolor[HTML]{F96346}} \color[HTML]{F1F1F1} +103\% \\
Replacement & Predicted worst & {\cellcolor[HTML]{91D28E}} \color[HTML]{000000} -42\% & {\cellcolor[HTML]{7FC97F}} \color[HTML]{000000} -47\% & {\cellcolor[HTML]{AB1016}} \color[HTML]{F1F1F1} +171\% & {\cellcolor[HTML]{FC8D6D}} \color[HTML]{F1F1F1} +78\% & {\cellcolor[HTML]{FB6C4C}} \color[HTML]{F1F1F1} +99\% \\
Replacement & Pred. worst ($\alpha = 2$) & {\cellcolor[HTML]{A4DA9E}} \color[HTML]{000000} -37\% & {\cellcolor[HTML]{66BD6F}} \color[HTML]{F1F1F1} -53\% & {\cellcolor[HTML]{B01217}} \color[HTML]{F1F1F1} +167\% & {\cellcolor[HTML]{FC9879}} \color[HTML]{000000} +72\% & {\cellcolor[HTML]{FB7050}} \color[HTML]{F1F1F1} +96\% \\
Prediction & RFC & {\cellcolor[HTML]{95D391}} \color[HTML]{000000} -41\% & {\cellcolor[HTML]{45AD5F}} \color[HTML]{F1F1F1} -61\% & {\cellcolor[HTML]{FC8969}} \color[HTML]{F1F1F1} +81\% & {\cellcolor[HTML]{F24734}} \color[HTML]{F1F1F1} +118\% & {\cellcolor[HTML]{FA6648}} \color[HTML]{F1F1F1} +102\% \\
Prediction & KNN & {\cellcolor[HTML]{BCE4B5}} \color[HTML]{000000} -29\% & {\cellcolor[HTML]{9ED798}} \color[HTML]{000000} -39\% & {\cellcolor[HTML]{FDCCB8}} \color[HTML]{000000} +39\% & {\cellcolor[HTML]{FCB398}} \color[HTML]{000000} +55\% & {\cellcolor[HTML]{FDC5AE}} \color[HTML]{000000} +43\% \\
Prediction & RBF & {\cellcolor[HTML]{A0D99B}} \color[HTML]{000000} -38\% & {\cellcolor[HTML]{43AC5E}} \color[HTML]{F1F1F1} -62\% & {\cellcolor[HTML]{FC9576}} \color[HTML]{000000} +73\% & {\cellcolor[HTML]{FCAF93}} \color[HTML]{000000} +58\% & {\cellcolor[HTML]{FCB69B}} \color[HTML]{000000} +54\% \\
Prediction & GP Classifier & {\cellcolor[HTML]{A5DB9F}} \color[HTML]{000000} -36\% & {\cellcolor[HTML]{53B466}} \color[HTML]{F1F1F1} -58\% & {\cellcolor[HTML]{FC8F6F}} \color[HTML]{000000} +77\% & {\cellcolor[HTML]{FC8161}} \color[HTML]{F1F1F1} +86\% & {\cellcolor[HTML]{FC9B7C}} \color[HTML]{000000} +70\% \\
Prediction & Variational GP & {\cellcolor[HTML]{9FD899}} \color[HTML]{000000} -38\% & {\cellcolor[HTML]{46AE60}} \color[HTML]{F1F1F1} -61\% & {\cellcolor[HTML]{FCAB8F}} \color[HTML]{000000} +60\% & {\cellcolor[HTML]{67000D}} \color[HTML]{F1F1F1} +259\% & {\cellcolor[HTML]{860811}} \color[HTML]{F1F1F1} +187\% \\
Prediction & MD GP & {\cellcolor[HTML]{A2D99C}} \color[HTML]{000000} -37\% & {\cellcolor[HTML]{3FA95C}} \color[HTML]{F1F1F1} -63\% & {\cellcolor[HTML]{FC8161}} \color[HTML]{F1F1F1} +85\% & {\cellcolor[HTML]{FC9E80}} \color[HTML]{000000} +67\% & {\cellcolor[HTML]{FC9D7F}} \color[HTML]{000000} +68\% \\
\bottomrule
\end{tabular}

